Predictive Encoding of Contextual Relationships for Perceptual Inference, Interpolation and Prediction

We propose a new neurally-inspired model that can learn to encode the global relationship context of visual events across time and space and to use the contextual information to modulate the analysis by synthesis process in a predictive coding framework. The model learns latent contextual representations by maximizing the predictability of visual events based on local and global contextual information through both top-down and bottom-up processes. In contrast to standard predictive coding models, the prediction error in this model is used to update the contextual representation but does not alter the feedforward input for the next layer, and is thus more consistent with neurophysiological observations. We establish the computational feasibility of this model by demonstrating its ability in several aspects. We show that our model can outperform state-of-art performances of gated Boltzmann machines (GBM) in estimation of contextual information. Our model can also interpolate missing events or predict future events in image sequences while simultaneously estimating contextual information. We show it achieves state-of-art performances in terms of prediction accuracy in a variety of tasks and possesses the ability to interpolate missing frames, a function that is lacking in GBM.

==> analysis.tex <==
\section{Analysis of the Model}\label{sec:analysis}

\subsection{Autoencoder Perspective}
The proposed model share some similarities with Autoencoder since they both use the prediction(reconstruction) error as the objective cost function during training. Fig.\ref{fig-RAE} shows the depiction of our model form an Autoencoder perspective. This model is similar to an Autoencoder but differs in three major aspects.
First, it only use the surround frames to ``predict'' a specific time frame, without using the information in a particular time frame itself -- this is important for fulfilling the function of interpolation and prediction.
Second, it uses the a set of contextual latent variables to ``gate'' the encoding process, using context to decide how the surround should be used to predict the current frames. Thus, it is better be called a predictive encoder model.
Third, during inference after learning parameters, Autoencoder rely solely on fast feed-forward computation, here in our model, our model use a new predictive coding model that can encodes relationship context to mediate fast top-down and bottom-up inference to accomplish interpolation and prediction.

\begin{figure}[h]
  \centering
  \includegraphics[scale=1]{fig-RAE}\\
  \caption{fig-RAE}\label{fig-RAE}
\end{figure}

\subsection{Factor Graph Perspective}
\subsection{Adaptive Receptive Field Perspective}







\iffalse
\subsection{Graphical Model Perspective}
\begin{figure}[h]
  \centering
  \includegraphics[scale=1]{fig-pgm}\\
  \caption{Probabilistic Graphical Model}
  \label{proba_graph_model}
\end{figure}

We can view our model as a graphical model as shown in Fig.\ref{proba_graph_model}. The joint distribution of $\boldsymbol{x}_{1...T}$ and $\boldsymbol{h}$ can be denoted as $P_{\boldsymbol \theta}(\boldsymbol{x}_{1...T}, \boldsymbol{h})$, where ${\boldsymbol \theta}$ is all the parameters. We will show that we are maximizing this joint distribution in both the learning and inference procedure.

\subsubsection{Learning the Parameters.}

As $P_{\boldsymbol \theta}(\boldsymbol{x}_{1...T}, \boldsymbol{h}) = P_{\boldsymbol \theta}(\boldsymbol{h} \big | \boldsymbol{x}_{1...T}) P_{\boldsymbol \theta}(\boldsymbol{x}_{1...T})$ and $P_{\boldsymbol \theta}(\boldsymbol{x}_{1...T})$ is constant when ${\boldsymbol \theta}$ fixed and $\boldsymbol{x}_{1...T}$ given, maximizing the joint distribution $P_{\boldsymbol \theta}(\boldsymbol{x}_{1...T}, \boldsymbol{h})$ is effectively the same as maximizing $P_{\boldsymbol \theta}(\boldsymbol{h} \big | \boldsymbol{x}_{1...T})$ . So in both the learning and inference procedure, $\boldsymbol{h}$ is determined by:

\begin{equation}
\label{infer_h_given_x_all}
\begin{aligned}
\boldsymbol{h}^*  = & \underset{\boldsymbol{h}}{\text{argmax }} P_{\boldsymbol \theta}(\boldsymbol{x}_{1...T}, \boldsymbol{h})
\end{aligned}
\end{equation}

, which we can prove that is the same as the optimization rule to determine $\boldsymbol{h}$ in our model.

We will show that our algorithm is actually maximizing the joint distribution, which is also the likelihood function of $\boldsymbol{\theta}$, $P_{\boldsymbol{\theta}}(\boldsymbol{X}, \boldsymbol{H})$ of all the data $\boldsymbol{X}=\{\boldsymbol{x}^{(1)}_{1...T},...,\boldsymbol{x}^{(m)}_{1...T}\}$ and all the corresponding latent variables $\boldsymbol{H}=\{\boldsymbol{h}^{(1)},...,\boldsymbol{h}^{(m)}\}$. As every data $\boldsymbol{x}^{(i)}_{1...T}$ is sampled i.i.d. from the unknown distribution $P(\boldsymbol{X})$. Maximizing the log-likelihood function to get $\boldsymbol{\theta}$ also means:

\begin{equation}
\label{training_in_PGM}
\begin{aligned}
\boldsymbol{\theta}^*  & = \underset{\boldsymbol{\theta}}{\text{argmax }} \mathcal{L}(\boldsymbol{\theta} {\big |} \boldsymbol{X, H} ) \\
                & = \underset{\boldsymbol{\theta}}{\text{argmax }} \underset{i} \sum \mathcal{L}(\boldsymbol{\theta} {\big |} \boldsymbol{x}^{(i)}, \boldsymbol{H}^{(i)} ) \\
                & = \underset{\boldsymbol{\theta}}{\text{argmin }} \underset{i} \sum {L(\boldsymbol{x}^{(i)}_{1...T}, \boldsymbol{h}^{(i)})}
%                & = \underset{\boldsymbol{W}}{\text{argmin}} \underset{i} \sum {L(\boldsymbol{x}^{(i)}_{1...T}, \boldsymbol{h}^{(i)})}
\end{aligned}
\end{equation}

The last equation is because we can prove our loss function $L(\boldsymbol{x}^{(i)}_{1...T}, \boldsymbol{h}^{(i)})$ is actually negative log-likelihood function.

\subsubsection{Inference.}

The inference procedure can also be viewed as maximum a posteriori estimation in the probabilistic graphical model. When we are inferencing with known type of partial observations, as the joint distribution $P_{\boldsymbol \theta}(\boldsymbol{x}_{1...T}, \boldsymbol{h})$ can be factorized as below:

\begin{equation}
\label{bayesian_infer}
\begin{aligned}
P_{\boldsymbol \theta}(\boldsymbol{x}_{1...T}, \boldsymbol{h})   = P_{\boldsymbol \theta}(\boldsymbol{x}_k, \boldsymbol{h} {\big |} \{\boldsymbol{x}_i {\big |} i \neq k\}) & \\ P_{\boldsymbol \theta}(\{\boldsymbol{x}_i {\big |} i \neq k\}) &
\end{aligned}
\end{equation}

So maximizing the joint distribution of all the data while fixed the observed part is effectively maximizing the joint distribution of unobserved part and latent variables, which will give us:

\begin{equation}
\label{infer_connection}
\begin{aligned}
\boldsymbol{x}^*_k, \boldsymbol{h}^*    & = \underset{\boldsymbol{x}_k, \boldsymbol{h}}{\text{argmax }} P_{\boldsymbol \theta}(\boldsymbol{x}_k, \boldsymbol{h} {\big |} \{\boldsymbol{x}_i {\big |} i \neq k\}) \\
                                        & = \underset{\boldsymbol{x}_k, \boldsymbol{h}}{\text{argmax }} P_{\boldsymbol \theta}(\boldsymbol{x}_{1...T}, \boldsymbol{h})\\
                                        & = \underset{\boldsymbol{x}_k, \boldsymbol{h}}{\text{argmin }} L(\boldsymbol{x}_{1...T}, \boldsymbol{h})
\end{aligned}
\end{equation}

And we can also show that alternatively optimizing w.r.t $\boldsymbol{x}_k$ and $\boldsymbol{k}$ is both optimizing the posterior probability, which indicates that the optimization will converge.


\subsection{Hierarchical Neural Network Perspective}
\begin{figure}[h]
  \centering
  \includegraphics[scale=1]{fig-nn}\\
  \caption{NN}\label{fig-nn}
\end{figure}
Our model can be viewed as a hierarchical neural network consisting of three different layers.
The first layer is the input sequence of images, the second layer $\boldsymbol{s}$ is the distributed representation of relationship between images and the third layer $\boldsymbol{h}$ is a sparse low-dimensional representation of the second layer $\boldsymbol{s}$.


While widely-used deep learning module like Restricted Boltzmann Machine(RBM) and Denoising AutoEncoder(DAE) are originally design to analysis images, this paper proposes an deep learning module that is designed to understand temporal information. More hidden layers can be used to make it a deep neural network which able to learn high-level features for recognition. We also develop unsupervised greedy pre-training algorithm which is crucial for learning deep architecture and fine-tuning is also possible given specific task and training data.

\subsection{Manifold Learning Perspective}
Our model can be viewed as a manifold representation in which unsupervised parameters learning and inference can be viewed as manifold learning and projection operation, respectively.

A manifold can be implicitly represented by defining distance to it. In our model, we can viewed the cost function defined in Eq.\eqref{cost_with_sparsity} as the distance measure.
\fi


==> description_tai.tex <==
\section{Description of the Model}

Conceptually, the model seeks to learn relationships between visual events in a temporal neighborhood to provide context for inference. That would be the relationships between different time frames in image sequences.  These relationships can be considered as temporal priors, a generalization of the typical `smoothness' constraint. We want to encode these temporal relationships in a set of latent variables as a form of temporal context, which can be used to infer missing frames as in interpolation, or can be used predicting the future frames.


\subsection{Cost Function Definition}
Let $\boldsymbol{x}_t \in \mathbb{R}^{N}, t = 1,2,...,T$ denote a sequence of images.  The objective cost function is defined as the sum of the reconstruction error for all the images in the sequence:

\begin{equation}\label{cost_func}
L(\boldsymbol{x}_{1...T}, \boldsymbol{h}) = \sum_t{loss(\boldsymbol{x}_t, \hat{\boldsymbol{x}}_t})
\end{equation}
where $loss(\cdot)$ is a loss function which is typically \emph{squared error} for real-valued images and $\hat{\boldsymbol{x}}_t$, which will be described later, is the reconstruction of $x_t$ by the latent variables based on the surrounding or preceding frames.

We further added a sparsity prior on the latent variables $h$, so the cost function in Eq.\eqref{cost_func} can be rewritten as:

\begin{equation}\label{cost_with_sparsity}
L(\boldsymbol{x}_{1...T}, \boldsymbol{h}) = \sum_t{\|\boldsymbol{x}_t - \hat{\boldsymbol{x}}_t\|_2^2} + \lambda\|\boldsymbol{h}\|_1
\end{equation}
where $\lambda>0$ is a parameter that balances the loss term and the regularization term. This cost function measures the degree the latent variables have captured the relationships inside the sequence of images.

This model is similar to an Autoencoder but differs in two major aspects, as shown in Figure \ref{fig-RAE}.  First, it only use the surround frames to `predict' a specific time frame, without using the information in a particular time frame itself -- this is important for fulfilling the function of interpolation and prediction. Second, it uses the a set of contextual latent variables to `gate' the encoding process, using context to decide how the surround should be used to predict the current frames. Thus, it is better be called a predictive encoder model.

\begin{figure}[h]
  \centering
  \includegraphics[scale=1]{fig-RAE}\\
  \caption{fig-RAE}\label{fig-RAE}
\end{figure}

{\bf We probably need to explain WHY standard DBN is not appropriate for encoding these priors or why is it can't do interpolation or prediction? Or is it? }

The model is now formulated as a factor graph, as shown in Figure \ref{fig-GM}. There is a set of learned $s$, each of which is connected to a subset of the input nodes (time frames), and to a set of latent contextual or relationship variables $h$. $s$ represents a relationship factor that relates visual patterns across multiple image frames. $h$ summarizes pattern-dependent relationship factor $s$ and represent  more abstract pattern-invariant relationship mapping in a lower low-dimensional space.

\begin{figure}[h]
  \centering
  \includegraphics[scale=1]{fig-GM}\\
  \caption{fig-GM}\label{fig-GM}
\end{figure}

The model seeks to learn a set of pattern basis functions $(\boldsymbol{W}_f^1,\boldsymbol{W}_f^2,...,\boldsymbol{W}_f^T)$, one for each image frame for each $s$ factor, where $f$ the index of a particular $s$ factor, as well as a set of contextual basis function $W_f^h$ that relates the latent contextual relationship variables ${\bf h}$ with that $s$ factor. In Roland's 3-way gated Boltzmann machine, T=2, and the cost function for a $s$ factor is the multiplication product $w^1 w^2 w^h x_1 x_2, h$. Our model structurally is similar to a T+1 way gated machine.

However, in our model, in order to have the capability to do interpolation and prediction, we do not assume we have full information or full confidence of all the visible units, and our model thus is based on synchrony-based multiplication as in the gated BM. Rather, we developed the concept of mutual predictability in which the various causes, including all the image frames and the context help to explain each other via the `relationship' factors learned based on the statistical of co-occurrence of visual events and context.

Formally, the prediction $\boldsymbol{x}_t$  from latent variables $\boldsymbol{h}$ and adjacent images is given by,

\begin{equation}\label{recon_x_given_s}
\hat{\boldsymbol{x}}_t = {(\boldsymbol{W}^t)}^{\mathrm{T}}((\sum_{i\in\mathcal{N}(t)}{{\frac{1}{|\mathcal{N}(t)|}}\boldsymbol{W}^i\boldsymbol{x}_i})\odot \boldsymbol{W}^h\boldsymbol{h})
\end{equation}
where $\mathcal{N}(t)$ defines the neighborhood of $t$-th image in the sequence {\bf This does not include image t, right?}, $|\cdot|$ denotes the size of a set and $\odot$ is element-wise multiplication.  $\boldsymbol{W}^t$ is the basis function of $t^{th}$ frame for the factors, and $(\sum_{i\in\mathcal{N}(t)}{{\frac{1}{|\mathcal{N}(t)|}}\boldsymbol{W}^i\boldsymbol{x}_i})$ is the average weighted input from the surrounding frames.  $\boldsymbol{W}^h\boldsymbol{h}$ represents the feedback from the context that weight the importance of each relationship factors to gate or select the the appropriate $s$ to achieve interpolation and prediction.

The information flow is best represented by a `neural' circuit diagram shown in Figure \ref{fig-NC}. This predictive encoder seeks to reconstruct a signal based purely on neighborhood and contextual information. It does put a greater burden on what the hidden variables can encode, forcing the hidden variables to learn the relationship between the image frames. {\bf I think there is still some conceptual issues on justification and motivation here бн maybe something is still missing.}  {\bf I can think whether it is worthwhile to connect it to neuroscience. We can say something in Motivation and Discussion. But one can't use ``neuroscience'' to justify it.  We can only evoke neuroscience to make it more interesting, maybe.}

\begin{figure}[h]
  \centering
  \includegraphics[scale=1]{fig-NC}\\
  \caption{fig-NC}\label{fig-NC}
\end{figure}

\subsection{Unsupervised Parameters Learning}

{\bf maybe add more details here.  add what parameters, $w, w^h$.  Update W, say given h, in Update h, say given W. etc.}


In this section, we will describe the algorithm to learn parameters in an unsupervised fashion while simultaneously estimate the latent variables for training data.
The training dataset contains $m$ sequences of images $\{\boldsymbol{x}^{(1)}_{1...T},...,\boldsymbol{x}^{(m)}_{1...T}\}$ and we suppose each sequence to be an i.i.d sample from unknown distribution. We denote the latent variables to be estimated for sequence $\boldsymbol{x}^{(i)}_{1...T}$ as $\boldsymbol{h}^{(i)}$.

Our goal is the following optimization problem:
\begin{equation}\label{optimization_learning}
\begin{aligned}
& \underset{\boldsymbol{W},\boldsymbol{h}}{\text{minimize}}
&& \sum_{i=1}^m{L(\boldsymbol{x}^{(i)}_{1...T}, \boldsymbol{h}^{(i)})}\\
\end{aligned}
\end{equation}

We update the $\boldsymbol{W}$ and $\boldsymbol{h}$ by minimize this function w.r.t the variables alternately.

\subsubsection{Update $\boldsymbol{W}$.}%(two choices now)

%(choice 1) Stochastic gradient descent (SGD).
%(choice 2)
We update $\boldsymbol{W}^{t}$ for different $t$ alternatively. Note that the optimization function is a linear least square w.r.t to $\boldsymbol{W}^{t}$ which have a global minimum with closed form solution. However, in practice, updating $\boldsymbol{W}^{t}$ with closed form solution is prohibitive since the dimensionality of $\boldsymbol{W}^{t}$ is too large(i.e. tens of thousands). We use L-BFGS algorithm which is an approximation of Newton's method to achieve global minimum efficiently. (AT LEAST faster than gradient descent, BUT there must be some work solving the specific problem of large-scale linear least squares.)

\subsubsection{Update $\boldsymbol{h}$.}

We update $\boldsymbol{h}$ by solving the optimization problems for each $\boldsymbol{h}^{(i)}$ independently:
\begin{equation}\label{optimization_update_h}
\begin{aligned}
& \underset{\boldsymbol{h}^{(i)}}{\text{minimize}}
\sum_t{\|\boldsymbol{x}^{(i)}_t - \hat{\boldsymbol{x}}^{(i)}_t\|_2^2} + \lambda\|\boldsymbol{h}^{(i)}\|_1\\
\end{aligned}
\end{equation}
where $\hat{\boldsymbol{x}}^{(i)}_t$ is a linear transformation of $\boldsymbol{h}^{(i)}$.

\subsection{Inference with Partial Observation}

{\bf It might be more elegant to absorb inference of  ``known type'' into ``unknown type''. known type can be called ``prediction'', unknown type can be called interpolation, or denoising.  For example if some frames got some noises and scratch, could you remove them.  For interpolation, can you formulate as ``prediction'' from both ends, if you known $k_1, k_2$, you can predict $k_3$,  if you know $k_5, k_4$, you can also predict $k_3$.  With two predictions as initial conditions, maybe you can find a better interpolation?}

There are two types of partial observation, in the first situation, we know which part is observed and what else should be estimated, for instance, inference of a specific image given other images in the sequence. In the second kind of situation, which part is unobserved is not known, part of the sequence may be corrupted or noisy, for instance, images sequence denoising.

\subsubsection{Inference with known type of partial observation.}
Inference with known type of partial observation refers to inference of an image given others in the sequence observed. This problem can be formulated as an optimization problem which simultaneously estimate latent variables $\boldsymbol{h}$ and unobserved image $\boldsymbol{x}_k, 1\leq k\leq T$:
\begin{equation}\label{optimization_known obser}
\begin{aligned}
& \underset{\boldsymbol{x}_k,\boldsymbol{h}}{\text{minimize}}
&& L(\boldsymbol{x}_{1...T}, \boldsymbol{h})\\
\end{aligned}
\end{equation}
This optimization problem can be solved efficiently by alternatively optimizing w.r.t $\boldsymbol{x}_k$ and $\boldsymbol{h}$, each of which is a linear least squares optimization and can be solved in one step.

\subsubsection{Inference with unknown type of partial observation.}
In some cases, all the images in the sequence are given but they may be noisy or corrupted. Makrov Random Field which considers the spatial smoothness is used to denoise for a single static image. Here, we show that our model can be used to do denoising task utilizing both spatial smoothness and temporal correspondence.

Similar to Markov Random Field, we formulate the denoising task which tries to reconstruct ``clean'' output $\boldsymbol{x}_{1...T}$ with corrupted data $\tilde{\boldsymbol{x}}_{1...T}$ as follows:
\begin{equation}\label{optimization_unknown obser}
\begin{aligned}
& \underset{\boldsymbol{x}_{1...T},\boldsymbol{h}}{\text{minimize}}
&& L(\boldsymbol{x}_{1...T}, \boldsymbol{h}) + \eta\sum_t{\|\tilde{\boldsymbol{x}}_{t} - \boldsymbol{x}_{t}\|^2_2}\\
\end{aligned}
\end{equation}
where $L(\boldsymbol{x}_{1...T}, \boldsymbol{h})$ is the temporal correspondence term, $\sum_t{\|\tilde{\boldsymbol{x}}_{t} - \boldsymbol{x}_{t}\|^2_2}$ is the data term and $\eta>0$ is a parameter that balances the correspondence term and the data term.


==> related_work.tex <==
\section{Related Work}\label{sec:related_work}

\noindent{\bf Bi-partite Networks}\hspace{2mm}
Bi-partite networks like Restricted Boltzmann Machines \cite{hinton2006fast}, auto-encoder networks \cite{bengio2007greedy}, ICA \cite{le2011ISA} and many others \cite{lee2008sparse,vincent2008extracting} have served as useful modules for building powerful hierarchical system such as deep belief nets for learning internal models of world for classification features.
The idea of convolution \cite{lecun1998gradient,lee2009convolutional} was used to extract features for larger spatial area using smaller shared networks.
The idea of recurrent \cite{sutskever2009recurrent,boulanger2012modeling} was used to model the temporal evolution of features for classification.
In those models, however, independent hidden variables interact with independent observable variables, such that there are no horizontal connections to explicitly model the relationship between observable variables.
The lack of their abilities to capture temporal or spatial relationships between visual events makes those models difficult to be used to interpolate missing events or predict future events, or to explain constructive or generative aspects of visual perception.

\noindent{\bf Gated Boltzmann Machine}\hspace{2mm}
The gated Boltzmann machine are fundamentally based on the idea of multiplicative interactions between observable variables.
The development on this model so far has centered on 3-way interaction \cite{susskind2011modeling,memisevic2011gradient} to relate two images.
Although the model may be modified to compute the square of the concatenation of more than two images to emulate multiplicative interactions, how to design more flexible interaction between more than two visual events based on their spatial or temporal structure remains an open question.
Additionally, the hidden variables of gated Boltzmann machine perform synchrony detection based on learned filters to relate images, however, the model can not simultaneously detect synchrony and interpolate missing events or predict future events.

To overcome the above limitations of 3-way gated Boltzmann machine, we propose a model considering more flexible multiplicative interaction based on spatial or temporal neighborhood structure of more than two visual events. The hidden variables gating those interactions are designed based on the idea of predictive coding that seeks to maximize mutual predictability which is more scalable for more than two images and capable of explaining constructive or generative aspects of visual perception.
It's worth mentioning that \citeauthor{MichalskiMK14} \shortcite{MichalskiMK14} applied gated machine for every two adjacent frames and assumed higher-order relationship to be constant thus propagated hidden variables though those gated machines. This method can be used for a specific type of inference, namely predicting future events but is still lacking in its abilities to interpolate or provide a model that can perform different types of inference in a unified framework.

